Local Refinement and Multilevel Preconditioning: Implementation and Numerical Experiments

In this paper, we examine a number of additive and multiplicative multilevel iterative methods and preconditioners in the setting of two-dimensional local mesh refinement. While standard multilevel methods are effective for uniform refinement-based discretizations of elliptic equations, they tend to be less effective for algebraic systems which arise from discretizations on locally refined meshes, losing their optimal behavior in both storage and computational complexity. Our primary focus here is on BPX-style additive and multiplicative multilevel preconditioners, and on various stabilizations of the additive and multiplicative hierarchical basis method (HB), and their use in the local mesh refinement setting. In this article, we describe in detail the implementation of these types of algorithms, including detailed discussions of the datastructures and traversal algorithms we employ for obtaining optimal storage and computational complexity in our implementations. We show how each of the algorithms can be implemented using standard datatypes available in languages such as C and FORTRAN, so that the resulting algorithms have optimal (linear) storage requirements, and so that the resulting multilevel method or preconditioner can be applied with optimal (linear) computational costs. Our implementations are performed in both C and MATLAB using the Finite Element ToolKit (FETK), an open source finite element software package. We finish the paper with a sequence of numerical experiments illustrating the effectiveness of a number of BPX and stabilized HB variants for several examples requiring local refinement.

==> app.tex <==
\section{Appendix: Highlights from The MCLite Implementation}

{\small

\begin{verbatim}
function [u]=multiplicative(b,lev,hb);
%%% Multiplicative methods: MG, M.BPX, HBMG, WMHBMG

%%% prolongation, stiffness, change of basis, one-ring
global P_12 P_23 P_34 P_45 A_1 A_2 A_3 A_4 A_5;
global level S_2 S_3 S_4 S_5 ONER_2 ONER_3 ONER_4 ONER_5;
global A_hb smthKey exactC bpx;

%%% get the stiffness matrix on this level
A = eval(['A_' num2str(lev)]);

if (lev == 1)
   if (exactC) u = A \ b; else u = b; end;
else
   ONER = eval(['ONER_' num2str(lev)]);

   %%% recover the dimensions
   P = eval(['P_' num2str(lev-1) num2str(lev)]);
   [r c] = size(P);

   %%% shorthand for the top and tail of vectors/matrices
   top_  = 1:c;
   tail_ = (c+1):r;

   if (hb)
      u = zeros(r,1);
      f = b;

      %%% Get the change of basis matrix for this level
      S = eval(['S_' num2str(lev)]);
      %%% Transform f into the HB basis
      f = f + S'*f;
      %%% pre-smoothing by symmetric Gauss-Seidel
      u = smooth_point(A_hb,u,f,smthKey,2,lev);
      %%% correct f using smoother result
      f(top_,1) = f(top_,1) - A_hb(top_,tail_)*u(tail_,1);
   else %%% mg/bpx
      u = zeros(c,1);
      d = zeros(r,1);
      if (bpx)
         d = smooth_point(A,d,b,smthKey,3,lev);
      else %%% mg
         d = smooth_point(A,d,b,smthKey,1,lev);
      end;

      %%% coarse grid defect restriction: f = P'*(b - A*d);
      if (bpx)
         f = b - A(:,ONER)*d(ONER);
      else %%% mg
         f = b - A*d;
      end
      
      f(top_,1) = f(top_,1) + P(tail_,:)'*f(tail_,1);
   end;

   %%% Recursion
   u(top_,1) = multiplicative(f(top_,1),lev-1,hb);

   if (hb)
      %%% correct f using the coarse solve result
      f(tail_,1) = f(tail_,1) - A_hb(tail_,top_)*u(top_,1);

      %%% post-smoothing by symmetric Gauss-Seidel
      u = smooth_point(A_hb,u,f,smthKey,2,lev);

      %%% transform u back into the nodal basis
      u = u + S*u;
   else %%% mg/bpx
      %%% interpolate result: u = P*u;
      u(tail_,1) =  P(tail_,:)*u(top_,1);

      if (bpx)
         u(ONER) = u(ONER) + d(ONER);
         u = smooth_point(A,u,b,smthKey,3,lev);
      else %%% mg
         u = u + d;
         u = smooth_point(A,u,b,smthKey,1,lev);
      end
end;


function [u]=additive(f,lev,hb);
%%% Additive methods: A.MG, BPX, HB, WMHB

%%% prolongation, stiffness, change of basis, one-ring
global P_12 P_23 P_34 P_45 A_1 A_2 A_3 A_4 A_5;
global S_2 S_3 S_4 S_5 ONER_2 ONER_3 ONER_4 ONER_5;
global A_hb smthKey exactC bpx;

%%% get the stiffness matrix on this level
A = eval(['A_' num2str(lev) ]);

if (lev == 1)
   if (exactC) u = A \ f; else u = f; end
else
   ONER = eval(['ONER_' num2str(lev)]);

   %%% recover the dimensions
   P = eval(['P_' num2str(lev-1) num2str(lev)]);
   [r c] = size(P);

   %%% shorthand for the top and tail of vectors/matrices
   top_  = 1:c;
   tail_ = (c+1):r;

   if (hb)
      u = zeros(r,1);

      %%% Get the change of basis matrix for this level
      S = eval(['S_' num2str(lev)]);
      %%% Transform f into the HB basis
      f = f + S'*f;
      %%% fine smoothing by symmetric Gauss-Seidel
      u = smooth_point(A_hb,u,f,smthKey,2,lev);
   else %%% additive MG
      u = zeros(c,1);
      d = zeros(r,1);
      %%% smoothing by symmetric Gauss-Seidel
      if (bpx)
         d = smooth_point(A,d,f,smthKey,3,lev);
      else %%% mg
         d = smooth_point(A,d,f,smthKey,1,lev);
      end;

      %%% coarse grid restriction: f = P'*f;
      f(top_,1) = f(top_,1) + P(tail_,:)'*f(tail_,1);
   end;

   %%% Recursion
   u(top_,1) = additive(f(top_,1),lev-1,hb);

   if (hb)
      %%% Transform u into the HB basis
      u = u + S*u;
   else
      %%% interpolate result: u = P*u;
      u(tail_,1) = P(tail_,:)*u(top_,1);
      if (bpx)
         u(ONER) = u(ONER) + d(ONER);
      else %%% mg
         u = u + d;
      end;
   end;
end;
\end{verbatim}
}


